Likelihood Landscapes: A Unifying Principle Behind Many Adversarial Defenses

Convolutional Neural Networks have been shown to be vulnerable to adversarial examples, which are known to locate in subspaces close to where normal data lies but are not naturally occurring and of low probability. In this work, we investigate the potential effect defense techniques have on the geometry of the likelihood landscape - likelihood of the input images under the trained model. We first propose a way to visualize the likelihood landscape leveraging an energy-based model interpretation of discriminative classifiers. Then we introduce a measure to quantify the flatness of the likelihood landscape. We observe that a subset of adversarial defense techniques results in a similar effect of flattening the likelihood landscape. We further explore directly regularizing towards a flat landscape for adversarial robustness.

==> sections/experiments.tex <==
\begin{figure}[!ht]
\captionsetup[subfloat]{farskip=2pt,captionskip=0.5pt}
\begin{center}
\subfloat[CIFAR10]{\label{fig:fig4a}\includegraphics[width=0.5\linewidth]{figures/f_cifar_norm_progress.png}}
\hfill
\subfloat[Fashion-MNIST]{\label{fig:fig4b}\includegraphics[width=0.5\linewidth]{figures/f_fmnist_norm_progress.png}}

\end{center}
   \caption{Progress of test norm}
\label{fig:fig4}
\end{figure}


\subsection{Experiment Setup}

To see the effectiveness of AmsReg, we run experiments on CIFAR-10 and Fashion-MNIST and compare against Adversarial training[] and Jacobian Regularization[]. We adopt three architectures including LeNet, DDNet and ResNet18. Each model is trained for 200 epochs using piecewise learning rate decay(i.e. decay ten-fold after the 100th epoch and the 150th epoch). All models are optimized using SGD with momentum, $\rho$ = 0.9.


\subsection{Results and Analysis}

\begin{table}[!ht]
\centering
\caption{CIFAR10}
\label{tbl:table1}
\begin{tabular}{lcccc}
\toprule
\makecell{\series Model} & \thead{Defense} & \thead{\Phi} & \thead{Clean Accuracy} & \thead{PGD Accuracy}  \\
\midrule
\makecell{DDNet} & {No Defense} & $13035.5$ & $91.45\%$ & $1.7\%$ \\
\makecell{DDNet} & {AT, $\epsilon$=3$\slash$255} & $2066.4$ & $85.90\%$ & $45.71\%$\\
\makecell{DDNet} & {Jacobian, $\lambda$=0.05} & $1692.6$ & $86.06\%$ & $18.31\%$  \\
\makecell{DDNet} & {AmsReg, $\lambda$=1} & $768.7$ & $85.45\%$ & $20.78\%$  \\
\hline
\makecell{ResNet18} & {No Defense} & $13974.3$ & $94.69\%$ & $0.1\%$ \\
\makecell{ResNet18} & {AT, $\epsilon$=3$\slash$255} & $1055.0$ & $85.32\%$ & $57.48\%$  \\
\makecell{ResNet18} & {Jacobian, $\lambda$=0.05} &  $1945.1$ & $82.28\%$ & $14.73\%$  \\
\makecell{ResNet18} & {AmsReg, $\lambda$=1} & $659.5$ & $86.94\%$ & $11.07\%$ \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!ht]
\centering
\caption{Fashion-MNIST}
\label{tbl:table2}
\begin{tabular}{lcccc}
\toprule
\makecell{\series Model} & \thead{Defense} & \thead{\Phi} & \thead{Clean Accuracy} & \thead{PGD Accuracy}  \\
\midrule
\makecell{LeNet} & {No Defense} & $9435.9$  & $91.53\%$ & $0.0\%$   \\
\makecell{LeNet} & {AT, $\epsilon$=10$\slash$255} & $1504.0$ & $89.35\%$ & $62.64\%$  \\
\makecell{LeNet} & {Jacobian, $\lambda$=0.01} & $1694.6$ & $88.76\%$ &$34.71\%$   \\
\makecell{LeNet} & {AmsReg, $\lambda$=0.5} & $378.1$ & $89.51\%$ & $34.04\%$  \\
\hline
\makecell{ResNet18} & {No Defense} & $12952.8$ & $93.75\%$ & $0.1\%$ \\
\makecell{ResNet18} & {AT, $\epsilon$=10$\slash$255} & $1794.9$ & $91.64\%$ & $65.24\%$  \\
\makecell{ResNet18} & {Jacobian, $\lambda$=0.01} & $1336.5$ & $91.39\%$ & $45.37\%$  \\
\makecell{ResNet18} & {AmsReg, $\lambda$=0.5} & $482.9$ & $91.49\%$ & $46.06\%$  \\
\bottomrule
\end{tabular}
\end{table}

As you can see, through AmsReg, we are able to train models that have better flatness than Jacobian regularization and Adversarial training. The AmsReg models have comparable adversarial robustness to that of Jacobian regularization, which is however significantly weaker than that of Adversarial training.

We did further analysis by looking at the flatness along the gradient direction instead of random directions. It's interesting that even though AmsReg is able to flatten out random directions better than adversarial training, adversarial training tends to flatten out in the gradient direction significantly better than AmsReg, which might be the reason why AmsReg is not able to match the adversarial robustness of adversarial training. Similarly,  Jaocbian regularization is also not able to flatten out along gradient direction well. We will leave the next step of flattening out worst-case directions for future work.

\begin{figure}[H]
\captionsetup[subfloat]{farskip=2pt,captionskip=0.5pt}
\begin{center}
\subfloat[Adversarial training with eps=5]{\label{fig:fig4a}\includegraphics[width=0.3\linewidth]{figures/f_cifar_grad_adv5.png}}
\hfill
\subfloat[AmsReg with lambda=1]{\label{fig:fig4b}\includegraphics[width=0.3\linewidth]{figures/f_cifar_grad_weighted1.png}}
\hfill
\subfloat[Jacobian regularization with lambda=0.1]{\label{fig:fig4b}\includegraphics[width=0.3\linewidth]{figures/f_cifar_grad_jaco01.png}}

\end{center}
   \caption{Likelihood landscapes}
\label{fig:fig6}
\end{figure}







==> space_saver.tex <==
% Some illegal space-saving macros
\parskip=3pt
\abovedisplayskip 3.0pt plus2pt minus2pt%
\belowdisplayskip \abovedisplayskip
\renewcommand{\baselinestretch}{0.98}



\newenvironment{packed_enum}{
\begin{enumerate}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}
{\end{enumerate}}

\newenvironment{packed_item}{
\begin{itemize}[leftmargin=*]
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{itemize}}

\newlength{\sectionReduceTop}
\newlength{\sectionReduceBot}
\newlength{\subsectionReduceTop}
\newlength{\subsectionReduceBot}
\newlength{\abstractReduceTop}
\newlength{\abstractReduceBot}
\newlength{\captionReduceTop}
\newlength{\captionReduceBot}
%\newlength{\nameReduceTop}
\newlength{\subsubsectionReduceTop}
\newlength{\subsubsectionReduceBot}

\newlength{\eqnReduceTop}
\newlength{\eqnReduceBot}

\newlength{\horSkip}
\newlength{\verSkip}

\newlength{\figureHeight}
\setlength{\figureHeight}{1.7in}

%\newlength{\figureFraction}
\setlength{\horSkip}{-.09in}
\setlength{\verSkip}{-.1in}
%\setlength{\figureFraction}{.195}


%
\setlength{\subsectionReduceTop}{-0.05in}
\setlength{\subsectionReduceBot}{-0.09in}
\setlength{\sectionReduceTop}{-0.10in}
\setlength{\sectionReduceBot}{-0.10in}
\setlength{\subsubsectionReduceTop}{-0.06in}
\setlength{\subsubsectionReduceBot}{-0.09in}
%
%
%\setlength{\figureHeight}{1.5in}
\setlength{\abstractReduceTop}{-0.05in}
\setlength{\abstractReduceBot}{-0.10in}
%
%

\setlength{\eqnReduceTop}{-0.05in}
\setlength{\eqnReduceBot}{-0.05in}

%\setlength{\nameReduceTop}{-0.05in}


\setlength{\captionReduceTop}{-0.14in}
\setlength{\captionReduceBot}{-0.12in}
%\setlength{\captionReduceBot}{-0.15in}

